Classical T Tauri stars: magnetic fields, coronae, and star-disc interactions

The magnetic fields of young stars set their coronal properties and control their spin evolution via the star-disc interaction and outflows. Using 14 magnetic maps of 10 classical T Tauri stars (CTTSs) we investigate their closed X-ray emitting coronae, their open wind-bearing magnetic fields, and the geometry of magnetospheric accretion flows. The magnetic fields of all the CTTSs are multipolar. Stars with simpler (more dipolar) large-scale magnetic fields have stronger fields, are slower rotators, and have larger X-ray emitting coronae compared to stars with more complex large-scale magnetic fields. The field complexity controls the distribution of open and closed field regions across the stellar surface, and strongly influences the location and shapes of accretion hot spots. However, the higher order field components are of secondary importance in determining the total unsigned open magnetic flux, which depends mainly on the strength of the dipole component and the stellar surface area. Likewise, the dipole component alone provides an adequate approximation of the disc truncation radius. For some stars, the pressure of the hot coronal plasma dominates the stellar magnetic pressure and forces open the closed field inside the disc truncation radius. This is significant as accretion models generally assume that the magnetic field has a closed geometry out to the inner disc edge.

==> Journals.tex <==
\newcommand{\aj}{{AJ}}			
\newcommand{\araa}{{Ann.\ Rev.\ Astron.\ Astrophys.}}		
\newcommand{\apj}{{ApJ}}			
\newcommand{\apjl}{{ApJ Lett.}}		
\newcommand{\apjs}{{ApJS}}		
\newcommand{\apss}{{Ap\&SS}}		
\newcommand{\aap}{{A\&A.}}		
\newcommand{\aapr}{{A\&A~Rev.}}		
\newcommand{\aaps}{{A\&AS}}		
\newcommand{\an}{{AN}}			
\newcommand{\azh}{{AZh}}			
\newcommand{\baas}{{BAAS}}		
\newcommand{\BAIC}{{Bull.\ Astron.\ Inst.\ Czech.}}		
\newcommand{\jrasc}{{JRASC}}		
\newcommand{\memras}{{MmRAS}}		
\newcommand{\mnras}{{MNRAS}}		
\newcommand{\pra}{{Phys.~Rev.~A}}	
\newcommand{\prb}{{Phys.~Rev.~B}}	
\newcommand{\prc}{{Phys.~Rev.~C}}	
\newcommand{\prd}{{Phys.~Rev.~D}}	
\newcommand{\pre}{{Phys.~Rev.~E}}	
\newcommand{\prl}{{Phys.~Rev.~Lett.}}	
\newcommand{\pasp}{{PASP}}		
\newcommand{\pasj}{{PASJ}}		
\newcommand{\qjras}{{QJRAS}}		
\newcommand{\skytel}{{S\&T}}		
\newcommand{\solphys}{{Solar~Phys.}}	
\newcommand{\sovast}{{Soviet~Ast.}}	
\newcommand{\ssr}{{Space~Sci.~Rev.}}	
\newcommand{\zap}{{ZAp}}			
\newcommand{\nat}{{Nature}}		
\newcommand{\iaucirc}{{IAU~Circ.}}
\newcommand{\aplett}{{Astrophys.~Lett.}}
\newcommand{\apspr}{{Astrophys.~Space~Phys.~Res.}}
\newcommand{\bain}{{Bull.~Astron.~Inst.~Netherlands}}
\newcommand{\fcp}{{Fund.~Cosmic~Phys.}}
\newcommand{\gca}{{Geochim.~Cosmochim.~Acta}}
\newcommand{\grl}{{Geophys.~Res.~Lett.}}
\newcommand{\GAFD}{{Geophys.~Astrophys.~Fluid~Dyn.}}
\newcommand{\jcp}{{J.~Chem.~Phys.}}	
\newcommand{\jgr}{{J.~Geophys.~Res.}}	
\newcommand{\jqsrt}{{J.~Quant.~Spec.~Radiat.~Transf.}}
\newcommand{\memsai}{{Mem.~Soc.~Astron.~Italiana}}
\newcommand{\nphysa}{{Nucl.~Phys.~A}}
\newcommand{\physrep}{{Phys.~Rep.}}
\newcommand{\physscr}{{Phys.~Scr}}
\newcommand{\planss}{{Planet.~Space~Sci.}}
\newcommand{\procspie}{{Proc.~SPIE}}
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao

==> mybib__Autosaved_ <==
\begin{thebibliography}{93}
\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi

\bibitem[{{Adams} \& {Gregory}(2012)}]{2012ApJ...744...55A}
{Adams} F.~C., {Gregory} S.~G., 2012, \apj, 744, 55

\bibitem[{{Alencar} {et~al}\mbox{.}(2010){Alencar}, {Teixeira},
  {Guimar{\~a}es}, {McGinnis}, {Gameiro}, {Bouvier}, {Aigrain}, {Flaccomio}, \&
  {Favata}}]{2010A&A...519A..88A}
{Alencar} S.~H.~P. {et~al.}, 2010, A\&A, 519, A88+

\bibitem[{{Altschuler} \& {Newkirk}(1969)}]{1969SoPh....9..131A}
{Altschuler} M.~D., {Newkirk} G., 1969, Solar Phys., 9, 131

\bibitem[{{Ardila} {et~al}\mbox{.}(2013){Ardila}, {Herczeg}, {Gregory},
  {Ingleby}, {France}, {Brown}, {Edwards}, {Johns-Krull}, {Linsky}, {Yang},
  {Valenti}, {Abgrall}, {Alexander}, {Bergin}, {Bethell}, {Brown}, {Calvet},
  {Espaillat}, {Hillenbrand}, {Hussain}, {Roueff}, {Schindhelm}, \&
  {Walter}}]{2013ApJS..207....1A}
{Ardila} D.~R. {et~al.}, 2013, \apjs, 207, 1

\bibitem[{{Arge} \& {Pizzo}(2000)}]{2000JGR...10510465A}
{Arge} C.~N., {Pizzo} V.~J., 2000, \jgr, 105, 10465

\bibitem[{{Argiroffi} {et~al}\mbox{.}(2011){Argiroffi}, {Flaccomio}, {Bouvier},
  {Donati}, {Getman}, {Gregory}, {Hussain}, {Jardine}, {Skelly}, \&
  {Walter}}]{2011A&A...530A...1A}
{Argiroffi} C. {et~al.}, 2011, \aap, 530, A1

\bibitem[{{Arzoumanian} {et~al}\mbox{.}(2011){Arzoumanian}, {Jardine},
  {Donati}, {Morin}, \& {Johnstone}}]{2011MNRAS.410.2472A}
{Arzoumanian} D., {Jardine} M., {Donati} J.-F., {Morin} J., {Johnstone} C.,
  2011, \mnras, 410, 2472

\bibitem[{{Bessolaz} {et~al}\mbox{.}(2008){Bessolaz}, {Zanni}, {Ferreira},
  {Keppens}, \& {Bouvier}}]{2008A&A...478..155B}
{Bessolaz} N., {Zanni} C., {Ferreira} J., {Keppens} R., {Bouvier} J., 2008,
  \aap, 478, 155

\bibitem[{{Bouvier} {et~al}\mbox{.}(2007){Bouvier}, {Alencar}, {Boutelier},
  {Dougados}, {Balog}, {Grankin}, {Hodgkin}, {Ibrahimov}, {Kun}, {Magakian}, \&
  {Pinte}}]{2007A&A...463.1017B}
{Bouvier} J. {et~al.}, 2007, \aap, 463, 1017

\bibitem[{{Bouvier} {et~al}\mbox{.}(1986){Bouvier}, {Bertout}, {Benz}, \&
  {Mayor}}]{1986A&A...165..110B}
{Bouvier} J., {Bertout} C., {Benz} W., {Mayor} M., 1986, \aap, 165, 110

\bibitem[{{Bouvier} {et~al}\mbox{.}(1999){Bouvier}, {Chelli}, {Allain},
  {Carrasco}, {Costero}, {Cruz-Gonzalez}, {Dougados}, {Fern{\'a}ndez},
  {Mart{\'{\i}}n}, {M{\'e}nard}, {Mennessier}, {Mujica}, {Recillas}, {Salas},
  {Schmidt}, \& {Wichmann}}]{1999A&A...349..619B}
{Bouvier} J. {et~al.}, 1999, \aap, 349, 619

\bibitem[{{Bouvier} {et~al}\mbox{.}(2003){Bouvier}, {Grankin}, {Alencar},
  {Dougados}, {Fern{\'a}ndez}, {Basri}, {Batalha}, {Guenther}, {Ibrahimov},
  {Magakian}, {Melnikov}, {Petrov}, {Rud}, \& {Zapatero
  Osorio}}]{2003A&A...409..169B}
{Bouvier} J. {et~al.}, 2003, \aap, 409, 169

\bibitem[{{Brickhouse} {et~al}\mbox{.}(2010){Brickhouse}, {Cranmer}, {Dupree},
  {Luna}, \& {Wolk}}]{2010ApJ...710.1835B}
{Brickhouse} N.~S., {Cranmer} S.~R., {Dupree} A.~K., {Luna} G.~J.~M., {Wolk}
  S., 2010, \apj, 710, 1835

\bibitem[{{Camenzind}(1990)}]{1990RvMA....3..234C}
{Camenzind} M., 1990, in Reviews in Modern Astronomy, Vol.~3, Reviews in Modern
  Astronomy, {G.~Klare}, ed., pp. 234--265

\bibitem[{{Chandrasekhar}(1961)}]{1961hhs..book.....C}
{Chandrasekhar} S., 1961, {Hydrodynamic and hydromagnetic stability}

\bibitem[{{Clarke} {et~al}\mbox{.}(1995){Clarke}, {Armitage}, {Smith}, \&
  {Pringle}}]{1995MNRAS.273..639C}
{Clarke} C.~J., {Armitage} P.~J., {Smith} K.~W., {Pringle} J.~E., 1995, \mnras,
  273, 639

\bibitem[{{Donati}(2001)}]{2001LNP...573..207D}
{Donati} J.-F., 2001, in Lecture Notes in Physics, Berlin Springer Verlag, Vol.
  573, Astrotomography, Indirect Imaging Methods in Observational Astronomy,
  {Boffin} H.~M.~J., {Steeghs} D., {Cuypers} J., eds., p. 207

\bibitem[{{Donati} {et~al}\mbox{.}(2011{\natexlab{a}}){Donati}, {Bouvier},
  {Walter}, {Gregory}, {Skelly}, {Hussain}, {Flaccomio}, {Argiroffi},
  {Grankin}, {Jardine}, {M{\'e}nard}, {Dougados}, \&
  {Romanova}}]{2011MNRAS.412.2454D}
{Donati} J.-F. {et~al.}, 2011{\natexlab{a}}, \mnras, 412, 2454

\bibitem[{{Donati} {et~al}\mbox{.}(2011{\natexlab{b}}){Donati}, {Gregory},
  {Alencar}, {Bouvier}, {Hussain}, {Skelly}, {Dougados}, {Jardine},
  {M{\'e}nard}, {Romanova}, \& {Unruh}}]{2011MNRAS.417..472D}
{Donati} J.-F. {et~al.}, 2011{\natexlab{b}}, \mnras, 417, 472

\bibitem[{{Donati} {et~al}\mbox{.}(2012){Donati}, {Gregory}, {Alencar},
  {Hussain}, {Bouvier}, {Dougados}, {Jardine}, {M{\'e}nard}, \&
  {Romanova}}]{2012MNRAS.425.2948D}
{Donati} J.-F. {et~al.}, 2012, \mnras, 425, 2948

\bibitem[{{Donati} {et~al}\mbox{.}(2011{\natexlab{c}}){Donati}, {Gregory},
  {Montmerle}, {Maggio}, {Argiroffi}, {Sacco}, {Hussain}, {Kastner}, {Alencar},
  {Audard}, {Bouvier}, {Damiani}, {G{\"u}del}, {Huenemoerder}, \&
  {Wade}}]{2011MNRAS.417.1747D}
{Donati} J.-F. {et~al.}, 2011{\natexlab{c}}, \mnras, 417, 1747

\bibitem[{{Donati} {et~al}\mbox{.}(2007){Donati}, {Jardine}, {Gregory},
  {Petit}, {Bouvier}, {Dougados}, {M{\'e}nard}, {Collier Cameron}, {Harries},
  {Jeffers}, \& {Paletou}}]{2007MNRAS.380.1297D}
{Donati} J.-F. {et~al.}, 2007, \mnras, 380, 1297

\bibitem[{{Donati} {et~al}\mbox{.}(2008{\natexlab{a}}){Donati}, {Jardine},
  {Gregory}, {Petit}, {Paletou}, {Bouvier}, {Dougados}, {M{\'e}nard},
  {Cameron}, {Harries}, {Hussain}, {Unruh}, {Morin}, {Marsden}, {Manset},
  {Auri{\`e}re}, {Catala}, \& {Alecian}}]{2008MNRAS.386.1234D}
{Donati} J.-F. {et~al.}, 2008{\natexlab{a}}, MNRAS, 386, 1234

\bibitem[{{Donati} {et~al}\mbox{.}(2008{\natexlab{b}}){Donati}, {Morin},
  {Petit}, {Delfosse}, {Forveille}, {Auri{\`e}re}, {Cabanac}, {Dintrans},
  {Fares}, {Gastine}, {Jardine}, {Ligni{\`e}res}, {Paletou}, {Velez}, \&
  {Th{\'e}ado}}]{2008MNRAS.390..545D}
{Donati} J.-F. {et~al.}, 2008{\natexlab{b}}, \mnras, 390, 545

\bibitem[{{Donati} {et~al}\mbox{.}(2010{\natexlab{a}}){Donati}, {Skelly},
  {Bouvier}, {Gregory}, {Grankin}, {Jardine}, {Hussain}, {M{\'e}nard},
  {Dougados}, {Unruh}, {Mohanty}, {Auri{\`e}re}, {Morin}, {Far{\`e}s}, \& {MAPP
  Collaboration}}]{2010MNRAS.409.1347D}
{Donati} J.-F. {et~al.}, 2010{\natexlab{a}}, \mnras, 409, 1347

\bibitem[{{Donati} {et~al}\mbox{.}(2010{\natexlab{b}}){Donati}, {Skelly},
  {Bouvier}, {Jardine}, {Gregory}, {Morin}, {Hussain}, {Dougados},
  {M{\'e}nard}, \& {Unruh}}]{2010MNRAS.402.1426D}
{Donati} J.-F. {et~al.}, 2010{\natexlab{b}}, \mnras, 402, 1426

\bibitem[{{Edwards} {et~al}\mbox{.}(1994){Edwards}, {Hartigan}, {Ghandour}, \&
  {Andrulis}}]{1994AJ....108.1056E}
{Edwards} S., {Hartigan} P., {Ghandour} L., {Andrulis} C., 1994, \aj, 108, 1056

\bibitem[{{Elsner} \& {Lamb}(1977)}]{1977ApJ...215..897E}
{Elsner} R.~F., {Lamb} F.~K., 1977, \apj, 215, 897

\bibitem[{{Getman} {et~al}\mbox{.}(2008){Getman}, {Feigelson}, {Broos},
  {Micela}, \& {Garmire}}]{2008ApJ...688..418G}
{Getman} K.~V., {Feigelson} E.~D., {Broos} P.~S., {Micela} G., {Garmire} G.~P.,
  2008, ApJ, 688, 418

\bibitem[{{Ghosh} \& {Lamb}(1979{\natexlab{a}})}]{1979ApJ...232..259G}
{Ghosh} P., {Lamb} F.~K., 1979{\natexlab{a}}, \apj, 232, 259

\bibitem[{{Ghosh} \& {Lamb}(1979{\natexlab{b}})}]{1979ApJ...234..296G}
{Ghosh} P., {Lamb} F.~K., 1979{\natexlab{b}}, \apj, 234, 296

\bibitem[{{Ghosh} {et~al}\mbox{.}(1977){Ghosh}, {Pethick}, \&
  {Lamb}}]{1977ApJ...217..578G}
{Ghosh} P., {Pethick} C.~J., {Lamb} F.~K., 1977, \apj, 217, 578

\bibitem[{{Grankin} {et~al}\mbox{.}(2008){Grankin}, {Bouvier}, {Herbst}, \&
  {Melnikov}}]{2008A&A...479..827G}
{Grankin} K.~N., {Bouvier} J., {Herbst} W., {Melnikov} S.~Y., 2008, \aap, 479,
  827

\bibitem[{{Gregory} \& {Donati}(2011)}]{2011AN....332.1027G}
{Gregory} S.~G., {Donati} J.-F., 2011, Astronomische Nachrichten, 332, 1027

\bibitem[{{Gregory} {et~al}\mbox{.}(2012){Gregory}, {Donati}, {Morin},
  {Hussain}, {Mayne}, {Hillenbrand}, \& {Jardine}}]{2012ApJ...755...97G}
{Gregory} S.~G., {Donati} J.-F., {Morin} J., {Hussain} G.~A.~J., {Mayne} N.~J.,
  {Hillenbrand} L.~A., {Jardine} M., 2012, \apj, 755, 97

\bibitem[{{Gregory} {et~al}\mbox{.}(2010){Gregory}, {Jardine}, {Gray}, \&
  {Donati}}]{2010RPPh...73l6901G}
{Gregory} S.~G., {Jardine} M., {Gray} C.~G., {Donati} J.-F., 2010, Reports on
  Progress in Physics, 73, 126901

\bibitem[{{Gregory} {et~al}\mbox{.}(2006){Gregory}, {Jardine}, {Simpson}, \&
  {Donati}}]{2006MNRAS.371..999G}
{Gregory} S.~G., {Jardine} M., {Simpson} I., {Donati} J.-F., 2006, \mnras, 371,
  999

\bibitem[{{Gregory} {et~al}\mbox{.}(2008){Gregory}, {Matt}, {Donati}, \&
  {Jardine}}]{2008MNRAS.389.1839G}
{Gregory} S.~G., {Matt} S.~P., {Donati} J.-F., {Jardine} M., 2008, \mnras, 389,
  1839

\bibitem[{{G{\"u}del} {et~al}\mbox{.}(2007){G{\"u}del}, {Briggs}, {Arzner},
  {Audard}, {Bouvier}, {Feigelson}, {Franciosini}, {Glauser}, {Grosso},
  {Micela}, {Monin}, {Montmerle}, {Padgett}, {Palla}, {Pillitteri}, {Rebull},
  {Scelsi}, {Silva}, {Skinner}, {Stelzer}, \&
  {Telleschi}}]{2007A&A...468..353G}
{G{\"u}del} M. {et~al.}, 2007, \aap, 468, 353

\bibitem[{{G{\"u}del} {et~al}\mbox{.}(2008){G{\"u}del}, {Skinner}, {Audard},
  {Briggs}, \& {Cabrit}}]{2008A&A...478..797G}
{G{\"u}del} M., {Skinner} S.~L., {Audard} M., {Briggs} K.~R., {Cabrit} S.,
  2008, \aap, 478, 797

\bibitem[{{Hartmann} \& {Stauffer}(1989)}]{1989AJ.....97..873H}
{Hartmann} L., {Stauffer} J.~R., 1989, \aj, 97, 873

\bibitem[{{Hu{\'e}lamo} {et~al}\mbox{.}(2008){Hu{\'e}lamo}, {Figueira},
  {Bonfils}, {Santos}, {Pepe}, {Gillon}, {Azevedo}, {Barman}, {Fern{\'a}ndez},
  {di Folco}, {Guenther}, {Lovis}, {Melo}, {Queloz}, \&
  {Udry}}]{2008A&A...489L...9H}
{Hu{\'e}lamo} N. {et~al.}, 2008, \aap, 489, L9

\bibitem[{{Hussain}(2012)}]{2012AN....333....4H}
{Hussain} G.~A.~J., 2012, Astronomische Nachrichten, 333, 4

\bibitem[{{Hussain} {et~al}\mbox{.}(2009){Hussain}, {Collier Cameron},
  {Jardine}, {Dunstone}, {Ramirez Velez}, {Stempels}, {Donati}, {Semel},
  {Aulanier}, {Harries}, {Bouvier}, {Dougados}, {Ferreira}, {Carter}, \&
  {Lawson}}]{2009MNRAS.398..189H}
{Hussain} G.~A.~J. {et~al.}, 2009, \mnras, 398, 189

\bibitem[{{Jardine} {et~al}\mbox{.}(2006){Jardine}, {Collier Cameron},
  {Donati}, {Gregory}, \& {Wood}}]{2006MNRAS.367..917J}
{Jardine} M., {Collier Cameron} A., {Donati} J.-F., {Gregory} S.~G., {Wood} K.,
  2006, \mnras, 367, 917

\bibitem[{{Jardine} \& {Unruh}(1999)}]{1999A&A...346..883J}
{Jardine} M., {Unruh} Y.~C., 1999, \aap, 346, 883

\bibitem[{{Jardine} {et~al}\mbox{.}(2013){Jardine}, {Vidotto}, {van
  Ballegooijen}, {Donati}, {Morin}, {Fares}, \&
  {Gombosi}}]{2013MNRAS.431..528J}
{Jardine} M., {Vidotto} A.~A., {van Ballegooijen} A., {Donati} J.-F., {Morin}
  J., {Fares} R., {Gombosi} T.~I., 2013, \mnras, 431, 528

\bibitem[{{Jardine} {et~al}\mbox{.}(2002){Jardine}, {Wood}, {Collier Cameron},
  {Donati}, \& {Mackay}}]{2002MNRAS.336.1364J}
{Jardine} M., {Wood} K., {Collier Cameron} A., {Donati} J.-F., {Mackay} D.~H.,
  2002, \mnras, 336, 1364

\bibitem[{{Jardine} {et~al}\mbox{.}(2008){Jardine}, {Gregory}, \&
  {Donati}}]{2008MNRAS.386..688J}
{Jardine} M.~M., {Gregory} S.~G., {Donati} J.-F., 2008, \mnras, 386, 688

\bibitem[{{Johns-Krull}(2007)}]{2007ApJ...664..975J}
{Johns-Krull} C.~M., 2007, \apj, 664, 975

\bibitem[{{Johns-Krull} {et~al}\mbox{.}(1999){Johns-Krull}, {Valenti}, \&
  {Koresko}}]{1999ApJ...516..900J}
{Johns-Krull} C.~M., {Valenti} J.~A., {Koresko} C., 1999, \apj, 516, 900

\bibitem[{{Johnstone} {et~al}\mbox{.}(2010){Johnstone}, {Jardine}, \&
  {Mackay}}]{2010MNRAS.404..101J}
{Johnstone} C., {Jardine} M., {Mackay} D.~H., 2010, \mnras, 404, 101

\bibitem[{{Johnstone}(2012)}]{2012PhDT........75J}
{Johnstone} C.~P., 2012, PhD thesis, University of St Andrews

\bibitem[{{Kastner} {et~al}\mbox{.}(2002){Kastner}, {Huenemoerder}, {Schulz},
  {Canizares}, \& {Weintraub}}]{2002ApJ...567..434K}
{Kastner} J.~H., {Huenemoerder} D.~P., {Schulz} N.~S., {Canizares} C.~R.,
  {Weintraub} D.~A., 2002, \apj, 567, 434

\bibitem[{{K\"{o}nigl}(1991)}]{1991ApJ...370L..39K}
{K\"{o}nigl} A., 1991, \apjl, 370, L39

\bibitem[{{Kulkarni} \& {Romanova}(2008)}]{2008MNRAS.386..673K}
{Kulkarni} A.~K., {Romanova} M.~M., 2008, \mnras, 386, 673

\bibitem[{{Kurosawa} \& {Romanova}(2013)}]{2013MNRAS.431.2673K}
{Kurosawa} R., {Romanova} M.~M., 2013, \mnras, 431, 2673

\bibitem[{{Lang} {et~al}\mbox{.}(2012){Lang}, {Jardine}, {Donati}, {Morin}, \&
  {Vidotto}}]{2012MNRAS.424.1077L}
{Lang} P., {Jardine} M., {Donati} J.-F., {Morin} J., {Vidotto} A., 2012,
  \mnras, 424, 1077

\bibitem[{{Long} {et~al}\mbox{.}(2011){Long}, {Romanova}, {Kulkarni}, \&
  {Donati}}]{2011MNRAS.413.1061L}
{Long} M., {Romanova} M.~M., {Kulkarni} A.~K., {Donati} J.-F., 2011, \mnras,
  413, 1061

\bibitem[{{Long} {et~al}\mbox{.}(2005){Long}, {Romanova}, \&
  {Lovelace}}]{2005ApJ...634.1214L}
{Long} M., {Romanova} M.~M., {Lovelace} R.~V.~E., 2005, \apj, 634, 1214

\bibitem[{{Long} {et~al}\mbox{.}(2008){Long}, {Romanova}, \&
  {Lovelace}}]{2008MNRAS.386.1274L}
{Long} M., {Romanova} M.~M., {Lovelace} R.~V.~E., 2008, MNRAS, 386, 1274

\bibitem[{{Lynden-Bell} \& {Pringle}(1974)}]{1974MNRAS.168..603L}
{Lynden-Bell} D., {Pringle} J.~E., 1974, \mnras, 168, 603

\bibitem[{{Mackay} {et~al}\mbox{.}(2004){Mackay}, {Jardine}, {Cameron},
  {Donati}, \& {Hussain}}]{2004MNRAS.354..737M}
{Mackay} D.~H., {Jardine} M., {Cameron} A.~C., {Donati} J.-F., {Hussain}
  G.~A.~J., 2004, MNRAS, 354, 737

\bibitem[{{Mahdavi} \& {Kenyon}(1998)}]{1998ApJ...497..342M}
{Mahdavi} A., {Kenyon} S.~J., 1998, \apj, 497, 342

\bibitem[{{McGregor} {et~al}\mbox{.}(2008){McGregor}, {Hughes}, {Arge}, \&
  {Owens}}]{2008JGRA..11308112M}
{McGregor} S.~L., {Hughes} W.~J., {Arge} C.~N., {Owens} M.~J., 2008, Journal of
  Geophysical Research (Space Physics), 113, 8112

\bibitem[{{Mohanty} \& {Shu}(2008)}]{2008ApJ...687.1323M}
{Mohanty} S., {Shu} F.~H., 2008, \apj, 687, 1323

\bibitem[{{Morin} {et~al}\mbox{.}(2008){Morin}, {Donati}, {Petit}, {Delfosse},
  {Forveille}, {Albert}, {Auri{\`e}re}, {Cabanac}, {Dintrans}, {Fares},
  {Gastine}, {Jardine}, {Ligni{\`e}res}, {Paletou}, {Ramirez Velez}, \&
  {Th{\'e}ado}}]{2008MNRAS.390..567M}
{Morin} J. {et~al.}, 2008, \mnras, 390, 567

\bibitem[{{Morin} {et~al}\mbox{.}(2010){Morin}, {Donati}, {Petit}, {Delfosse},
  {Forveille}, \& {Jardine}}]{2010MNRAS.407.2269M}
{Morin} J., {Donati} J.-F., {Petit} P., {Delfosse} X., {Forveille} T.,
  {Jardine} M.~M., 2010, \mnras, 407, 2269

\bibitem[{{Nguyen} {et~al}\mbox{.}(2009){Nguyen}, {Jayawardhana}, {van
  Kerkwijk}, {Brandeker}, {Scholz}, \& {Damjanov}}]{2009ApJ...695.1648N}
{Nguyen} D.~C., {Jayawardhana} R., {van Kerkwijk} M.~H., {Brandeker} A.,
  {Scholz} A., {Damjanov} I., 2009, \apj, 695, 1648

\bibitem[{{Pillitteri} {et~al}\mbox{.}(2010){Pillitteri}, {Sciortino},
  {Flaccomio}, {Stelzer}, {Micela}, {Damiani}, {Testi}, {Montmerle}, {Grosso},
  {Favata}, \& {Giardino}}]{2010A&A...519A..34P}
{Pillitteri} I. {et~al.}, 2010, \aap, 519, A34

\bibitem[{{Preibisch} {et~al}\mbox{.}(2005){Preibisch}, {Kim}, {Favata},
  {Feigelson}, {Flaccomio}, {Getman}, {Micela}, {Sciortino}, {Stassun},
  {Stelzer}, \& {Zinnecker}}]{2005ApJS..160..401P}
{Preibisch} T. {et~al.}, 2005, \apjs, 160, 401

\bibitem[{{Reiners}(2011)}]{2011ASPC..448..255R}
{Reiners} A., 2011, in Astronomical Society of the Pacific Conference Series,
  Vol. 448, 16th Cambridge Workshop on Cool Stars, Stellar Systems, and the
  Sun, {Johns-Krull} C., {Browning} M.~K., {West} A.~A., eds., p. 255

\bibitem[{{Riley} {et~al}\mbox{.}(2006){Riley}, {Linker}, {Miki{\'c}},
  {Lionello}, {Ledvina}, \& {Luhmann}}]{2006ApJ...653.1510R}
{Riley} P., {Linker} J.~A., {Miki{\'c}} Z., {Lionello} R., {Ledvina} S.~A.,
  {Luhmann} J.~G., 2006, \apj, 653, 1510

\bibitem[{{Roberge} {et~al}\mbox{.}(2005){Roberge}, {Weinberger}, \&
  {Malumuth}}]{2005ApJ...622.1171R}
{Roberge} A., {Weinberger} A.~J., {Malumuth} E.~M., 2005, \apj, 622, 1171

\bibitem[{{Robrade} \& {Schmitt}(2006)}]{2006A&A...449..737R}
{Robrade} J., {Schmitt} J.~H.~M.~M., 2006, \aap, 449, 737

\bibitem[{{Romanova} {et~al}\mbox{.}(2011){Romanova}, {Long}, {Lamb},
  {Kulkarni}, \& {Donati}}]{2011MNRAS.411..915R}
{Romanova} M.~M., {Long} M., {Lamb} F.~K., {Kulkarni} A.~K., {Donati} J.-F.,
  2011, \mnras, 411, 915

\bibitem[{{Romanova} {et~al}\mbox{.}(2004){Romanova}, {Ustyugova}, {Koldoba},
  \& {Lovelace}}]{2004ApJ...610..920R}
{Romanova} M.~M., {Ustyugova} G.~V., {Koldoba} A.~V., {Lovelace} R.~V.~E.,
  2004, \apj, 610, 920

\bibitem[{{Romanova} {et~al}\mbox{.}(2003){Romanova}, {Ustyugova}, {Koldoba},
  {Wick}, \& {Lovelace}}]{2003ApJ...595.1009R}
{Romanova} M.~M., {Ustyugova} G.~V., {Koldoba} A.~V., {Wick} J.~V., {Lovelace}
  R.~V.~E., 2003, \apj, 595, 1009

\bibitem[{{Rosenfeld} {et~al}\mbox{.}(2012){Rosenfeld}, {Qi}, {Andrews},
  {Wilner}, {Corder}, {Dullemond}, {Lin}, {Hughes}, {D'Alessio}, \&
  {Ho}}]{2012ApJ...757..129R}
{Rosenfeld} K.~A. {et~al.}, 2012, \apj, 757, 129

\bibitem[{{Schatten} {et~al}\mbox{.}(1969){Schatten}, {Wilcox}, \&
  {Ness}}]{1969SoPh....6..442S}
{Schatten} K.~H., {Wilcox} J.~M., {Ness} N.~F., 1969, \solphys, 6, 442

\bibitem[{{Semel}(1989)}]{1989A&A...225..456S}
{Semel} M., 1989, \aap, 225, 456

\bibitem[{{Stassun} {et~al}\mbox{.}(2006){Stassun}, {van den Berg},
  {Feigelson}, \& {Flaccomio}}]{2006ApJ...649..914S}
{Stassun} K.~G., {van den Berg} M., {Feigelson} E., {Flaccomio} E., 2006, \apj,
  649, 914

\bibitem[{{Stelzer} \& {Schmitt}(2004)}]{2004A&A...418..687S}
{Stelzer} B., {Schmitt} J.~H.~M.~M., 2004, \aap, 418, 687

\bibitem[{{Stempels} \& {Piskunov}(2003)}]{2003A&A...408..693S}
{Stempels} H.~C., {Piskunov} N., 2003, \aap, 408, 693

\bibitem[{{Torres} {et~al}\mbox{.}(2003){Torres}, {Guenther}, {Marschall},
  {Neuh{\"a}user}, {Latham}, \& {Stefanik}}]{2003AJ....125..825T}
{Torres} G., {Guenther} E.~W., {Marschall} L.~A., {Neuh{\"a}user} R., {Latham}
  D.~W., {Stefanik} R.~P., 2003, \aj, 125, 825

\bibitem[{{van Ballegooijen} {et~al}\mbox{.}(1998){van Ballegooijen},
  {Cartledge}, \& {Priest}}]{1998ApJ...501..866V}
{van Ballegooijen} A.~A., {Cartledge} N.~P., {Priest} E.~R., 1998, ApJ, 501,
  866

\bibitem[{{Vrba} {et~al}\mbox{.}(1989){Vrba}, {Rydgren}, {Chugainov},
  {Shakovskaia}, \& {Weaver}}]{1989AJ.....97..483V}
{Vrba} F.~J., {Rydgren} A.~E., {Chugainov} P.~F., {Shakovskaia} N.~I., {Weaver}
  W.~B., 1989, \aj, 97, 483

\bibitem[{{Vrba} {et~al}\mbox{.}(1986){Vrba}, {Rydgren}, {Chugainov},
  {Shakovskaia}, \& {Zak}}]{1986ApJ...306..199V}
{Vrba} F.~J., {Rydgren} A.~E., {Chugainov} P.~F., {Shakovskaia} N.~I., {Zak}
  D.~S., 1986, \apj, 306, 199

\bibitem[{{Walter} \& {Kuhi}(1981)}]{1981ApJ...250..254W}
{Walter} F.~M., {Kuhi} L.~V., 1981, \apj, 250, 254

\bibitem[{{Wang}(1996)}]{1996ApJ...465L.111W}
{Wang} Y.-M., 1996, \apjl, 465, L111

\bibitem[{{Wang} \& {Sheeley}(1990)}]{1990ApJ...355..726W}
{Wang} Y.-M., {Sheeley}, Jr. N.~R., 1990, \apj, 355, 726

\bibitem[{{Wang} {et~al}\mbox{.}(1997){Wang}, {Sheeley}, {Hawley}, {Kraemer},
  {Brueckner}, {Howard}, {Korendyke}, {Michels}, {Moulton}, {Socker}, \&
  {Schwenn}}]{1997ApJ...485..419W}
{Wang} Y.-M. {et~al.}, 1997, \apj, 485, 419

\bibitem[{{Weise} {et~al}\mbox{.}(2010){Weise}, {Launhardt}, {Setiawan}, \&
  {Henning}}]{2010A&A...517A..88W}
{Weise} P., {Launhardt} R., {Setiawan} J., {Henning} T., 2010, \aap, 517, A88

\end{thebibliography}

